Evaluating Self-Supervised Learning via Risk Decomposition

Self-supervised learning (SSL) pipelines differ in many design choices such as the architecture, augmentations, or pretraining data. Yet SSL is typically evaluated using a single metric: linear probing on ImageNet. This does not provide much insight into why or when a model is better, now how to improve it. To address this, we propose an SSL risk decomposition, which generalizes the classical supervised approximation-estimation decomposition by considering errors arising from the representation learning step. Our decomposition consists of four error components: approximation, representation usability, probe generalization, and encoder generalization. We provide efficient estimators for each component and use them to analyze the effect of 30 design choices on 169 SSL vision models evaluated on ImageNet. Our analysis gives valuable insights for designing and using SSL models. For example, it highlights the main sources of error and shows how to improve SSL in specific settings (full- vs few-shot) by trading off error components. All results and pretrained models are at https://github.com/YannDubs/SSL-Risk-Decomposition.

==> figures/algorithms/main_estimationt.tex <==
\begin{minipage}{0.99\textwidth}
 \centering
\newcommand{\vspacing}{$\vphantom{\int_{i}^t}$} %$\vphantom{\sum_{i}^t}$
\begin{algorithm}[H]
\caption{Estimating risk components for representation learning}
\label{alg:components}
\begin{algorithmic}[1]
\Require{Encoders $\Phi$, probes $\Qz$, train $\Stask{}$ and test $\Ste$ sets, algorithms $\algrep{},\algsup{}$, eval loss $\ell$. }
%
\Function{SupRisk}{$\Qz, \ \mathcal{D}_{tr}, \ \mathcal{D}_{te},\ell$ }
\State \vspacing $\pred{\mathcal{D}_{tr}} \leftarrow \algsup(\hp{\mathcal{D}_{tr}}) \in \Qz$ \Comment{Supervised training}
\State \Return{$\frac{1}{|\mathcal{D}_{te}|} \sum_{(x,y) \in \mathcal{D}_{te}} \ell(y, \pred{\mathcal{D}_{tr}}(x))$} \Comment{Empirical risk}
 \EndFunction
 %
% \Procedure{decomposition}{}
\State \vspacing $\enc{}  \leftarrow  \algrep(\ppre) \in \Phi$ \Comment{Pretrain encoder}
\State \vspacing  $\hrFF{} \leftarrow  \Call{SupRisk}{\Phi \circ \Qz, \Stask, \Stask}$ \Comment{Supervised training risk}
\State \vspacing $\Senc{\enc{}} \leftarrow [(\enc{}(x),y) \text{ for } x,y \text{ in } \Stask]$
\State \vspacing $\Steenc{\enc{}} \leftarrow [(\enc{}(x),y) \text{ for } x,y \text{ in } \Ste]$
\Comment{Featurize data}
\State \vspacing $\Ssubenc{\enc{}} \leftarrow \mathrm{subset}(\Senc{\enc{}}, n=\mathrm{len}(\Steenc{\enc{}})$ 
\State \vspacing std\smallunderscore risk $ \leftarrow  \Call{SupRisk}{\Qz, \Senc{\enc{}}, \Steenc{\enc{}}}$ \Comment{Standard aggregated risk}
\State  $\hrAF \leftarrow  \Call{SupRisk}{\Q, \Senc{\enc{}}, \Senc{\enc{}}}$ \Comment{Risk without generalization}
\State \vspacing $\hrAS  \leftarrow  \Call{SupRisk}{\Qz, \Senc{\enc{}} \setminus \Ssubenc{\enc{}}, \Ssubenc{\enc{}}}$ \Comment{Only predictor generalization}
\State \vspacing $\hrUS \leftarrow  \Call{SupRisk}{\Qz, \Senc{\enc{}} \setminus \Ssubenc{\enc{}}, \Steenc{\enc{}}}$ \Comment{Both encoder and predictor gen.}
\State $\heA \leftarrow \hrFF$ \Comment{Discards constant $\brisk$ for approx. error}
\State $\heR \leftarrow \hrAF - \hrFF$ \Comment{Representation usability}
\State $\heP \leftarrow \hrAS - \hrAF$ \Comment{Predictor's generalization}
\State $\heE \leftarrow \hrUS - \hrAS$ \Comment{Encoder's generalization}
\State  \Return \vspacing std\smallunderscore risk,  $\heA$, $\heR$, $\heP$, $\heE$
 %\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{minipage}


==> figures/architecture/family_shapt.tex <==
\begin{figure}[h]
\centering
%\vspace*{-1em}
\includegraphics[width=\linewidth]{figures/architecture/family_shap.pdf}
%\vspace*{-2em}
\caption{
Impact of the architecture's family  (color) on risk components and aggregated full- or few-shot risk.
Lower SHAP values (x-axis) are better as Y-axis are errors.
% Impact of the architecture's family (color) on usability, probe generalization, and aggregated risk in the full- and few-shot setting.
% Impact is measured by SHAP values (x-axis).
% Lower is better as it decreases the risk.
}    \label{fig:architecture:family_shap}
\end{figure}

==> figures/architecture/size_shapt.tex <==
\begin{figure}[h]
\centering
%\vspace*{-1em}
\includegraphics[width=\linewidth]{figures/architecture/size_shap.pdf}
%\vspace*{-2em}
\caption{
Impact of the number of parameters (color) on risk components and aggregated full- or few-shot risk.
Lower SHAP values (x-axis) are better as x-axis are errors.
% Impact of the number of parameters (color) on usability, probe generalization, and aggregated risk in the full- and few-shot setting.
% Impact is measured by SHAP values (x-axis).
% Lower is better as it decreases the risk.
}    \label{fig:architecture:size_shap}
\end{figure}

==> figures/nviews/main_nviews_controlledt.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/nviews/controlled.pdf}
\caption{
Effect of the number of multicrops on usability and probe generalization error, when all other hyperparameters are kept the same. 
Each color shows a specific model.
}    \label{appcs:fig:nviews:main_controlled}
\vspace{-1em}
\end{figure}

==> figures/nviews/main_nviews_shapt.tex <==
\begin{figure}[h]
\centering
%\vspace*{-1em}
\includegraphics[width=\linewidth]{figures/nviews/main_shap.pdf}
%\vspace*{-2em}
\caption{
Impact of the number of multicrops  (color) on risk components and aggregated full- or few-shot risk.
Lower SHAP values (x-axis) are better as Y-axis are errors.
% Impact of the number of multicrops (color) on usability, probe generalization, and aggregated risk in the full- and few-shot setting.
% Impact is measured by SHAP values (x-axis).
% Lower is better as it decreases the risk.
}    \label{fig:nviews:main_shap}
\end{figure}

==> figures/nviews/nviews_controlledt.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/nviews/nviews_controlled.pdf}
    \caption{
    Effect of the number of multicrops on usability and probe generalization error, when all other hyperparameters are kept the same. 
    Each color shows a specific model.
}    \label{appcs:fig:nviews:controlled}
\end{figure}

==> figures/projection/proj_controlledt.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/projection/proj_controlled.pdf}
    \caption{
    Effect of the projection head on usability and probe generalization error, when all other hyperparameters are kept the same. 
    Each color shows a specific model.
}    \label{appcs:fig:projection:controlled}
\end{figure}

==> figures/projection/projection_shapt.tex <==
\begin{figure}[h]
\centering
%\vspace*{-1em}
\includegraphics[width=\linewidth]{figures/projection/projection_shap.pdf}
%\vspace*{-2em}
\caption{
Impact of the projection's architecture  (color) on risk components and aggregated full- or few-shot risk.
Lower SHAP values (x-axis) are better as Y-axis are errors.
%Impact of the projection's architecture (color) on usability, probe generalization, and aggregated risk in the full- and few-shot setting.
%Impact is measured by SHAP values (x-axis).
%Lower is better as it decreases the risk.
}    \label{fig:projection:projection_shap}
\end{figure}

==> tables/all_encoders.tex <==
\begin{table}[h]
\caption{
\small
.\texttt{Other} specifies other arguments, in particular \texttt{d:} specifies the data (other than IN1k),  \texttt{m:} specifies the number of multi crops ( 2 for the standard $2 \times 224$, 6 for $2\times 160+4\times 96$, and 8 for $2\times 224+6\times 224$) \texttt{p:} specifies the projection head.
\texttt{+ft} denotes supervised finetuning on the pretraining data.
}
\end{table}
%
\begin{table}
\ContinuedFloat
\begin{subtable}[h]{\textwidth}
\begin{scriptsize}
\begin{center}
%\settowidth\rotheadsize{Cntr}
\caption{Predicting transforms}
\label{table:all_encoders_gen}
\begin{tabular}{lllllrrrrrrr}
\toprule
&  &  &  &  &  &   \multicolumn{4}{c}{Risk decomposition}  \\
\cmidrule(lr){7-10}\
  & Other & Arch. & Batch & Ep. & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$ \\ 
\midrule 
  (?) Color.  
 & d: IN1K  & RN50 & 640 & 28 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 (?) Color.  
 &  d: IN22K & RN50 & 640 & 28 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
\midrule[0.1pt]
RotNet & d: IN1K  & RN50 & 256 & 105 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$\\
 RotNet & d: IN22K & RN50 & 256 & 105 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$\\
\midrule[0.1pt]
Jigsaw & d: IN1K  & RN50 & 256 & 90 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$\\
 Jigsaw & d: IN22K & RN50 & 256 & 90 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$\\
\bottomrule
\end{tabular}
\end{center}
\end{scriptsize}
\end{subtable}
\end{table}
%
\begin{table}
\ContinuedFloat
 \begin{subtable}[h]{\textwidth}
\begin{scriptsize}
\begin{center}
\caption{Contrastive}
\label{table:all_encoders_contr}
\begin{tabular}{lllllrrrrrrr}
\toprule
&  &  &  &  &  &   \multicolumn{4}{c}{Risk decomposition}  \\
\cmidrule(lr){7-10}\
  & Other & Arch. & Batch & Ep. & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$ \\ 
\midrule 
 NPID  &  & RN50 & 256 & 200 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 NPID\textsuperscript{++}  &  & RN50 & 1024 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 NPID\textsuperscript{++}  &  & RN50w2 & 1024 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
\midrule[0.1pt]
 PIRL   & p: lin & RN50 & 1024 & 200 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
 PIRL   & p: lin & RN50 & 1024 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
 PIRL  & p: mlp & RN50 & 1024 & 200 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
 PIRL   & p: mlp & RN50 & 1024 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
\midrule[0.1pt]
 SimCLR  &  & RN50 & 512 & 100 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 SimCLR  &  & RN50 & 4096 & 100 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 SimCLR  &  & RN50 & 4096 & 200 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 SimCLR  &  & RN50 & 4096 & 400 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 SimCLR  &  & RN50 & 4096 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 SimCLR  &  & RN50 & 4096 & 1000 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 SimCLR  &  & RN50w2 & 4096 & 100 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 SimCLR  &  & RN50w2 & 4096 & 1000 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 SimCLR  &  & RN50w4 & 4096 & 1000 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 SimCLR  &  & RN101 & 4096 & 100 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
 SimCLR  &  & RN101 & 4096 & 1000 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
\midrule[0.1pt]
 CLIP   & d: CLIP & RN50 & 32,768 & 32 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ \\
  CLIP   & d: CLIP & RN50x4 & 32,768 & 32 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$
\\
  CLIP   & d: CLIP & RN50x16 & 32,768 & 32 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$
\\
  CLIP   & d: CLIP & RN50x64 & 32,768 & 32 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$
\\
  CLIP   & d: CLIP & RN101 & 32,768 & 32 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$
\\  
CLIP   & d: CLIP & ViT-B32 & 32,768 & 32 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$
\\
CLIP   & d: CLIP & ViT-B16 & 32,768 & 32 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$
\\
CLIP   & d: CLIP & ViT-L14 & 32,768 & 32 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$
\\
\bottomrule
\end{tabular}
\end{center}
\end{scriptsize}
\end{subtable}
\end{table}
%
\begin{table}
\ContinuedFloat
 \begin{subtable}[h]{\textwidth}
\begin{scriptsize}
\begin{center}
\caption{Distillating ISSL}
\label{table:all_encoders_dist}
\begin{tabular}{lllllrrrrrrr}
\toprule
&  &  &  &  &  &   \multicolumn{4}{c}{Risk decomposition}  \\
\midrule(lr){7-10}\
  & Other & Arch. & Batch & Ep. & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$ \\ 
\midrule 
 Clusterfit  &  & RN50 & 256 & 105 & Agg.  & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
\midrule[0.1pt]
 DeepC.v2  & m: 2 & RN50 &  & 400 & Agg.  & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
 DeepC.v2  & m: 6 & RN50 &  & 400 & Agg.  & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
\midrule[0.1pt]
 Barlow Tw.  &   & RN50 & 2048 & 300 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
Barlow Tw.  &   & RN50 & 2048 & 1000 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$	& $\eP'$ &  $\eE'$ \\
\midrule[0.1pt]
 SWAV  & m: 2 & RN50 & 4096 & 400 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
SWAV  & m: 8 & RN50 & 256 & 200 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 SWAV  & m: 8 & RN50 & 256 & 400 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 SWAV  & m: 8 & RN50 & 4096 & 100 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 SWAV  & m: 8 & RN50 & 4096 & 200 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 SWAV  & m: 8 & RN50 & 4096 & 400 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 SWAV  & m: 8 & RN50 & 4096 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 SWAV  & m: 8 & RN50w2 & 4096 & 400 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 SWAV  & m: 8 & RN50w4 & 2560 & 400 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 SWAV  & m: 8 & RN50w4 & 2560 & 300 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
\midrule[0.1pt]
 SimSiam  &  & RN50 & 256 & 100 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
\midrule[0.1pt]
 MOCOv3  &  & RN50 & 4096 & 100 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 MOCOv3  &  & RN50 & 4096 & 300 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 MOCOv3  &  & RN50 & 4096 & 1000 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 MOCOv3  &  & ViT-S16 & 4096 & 300 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
 MOCOv3  &  & ViT-B16 & 4096 & 300 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$	 \\
\midrule[0.1pt]
 DINO &  & RN50 & 4080 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
 DINO &  & ViT-S16 & 1024 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
 DINO &  & ViT-S8 & 1024 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
 DINO &  & ViT-B16 & 1024 & 400 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
 DINO &  & ViT-B8 & 1056 & 300 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$\\
\bottomrule
\end{tabular}
\end{center}
\end{scriptsize}
\end{subtable}
\end{table}
%
\begin{table}
\ContinuedFloat
 \begin{subtable}[h]{\textwidth}
\begin{scriptsize}
\begin{center}
\caption{Masking}
\label{table:all_encoders_mask}
\begin{tabular}{lllllrrrrrrr}
\toprule
&  &  &  &  &  &   \multicolumn{4}{c}{Risk decomposition}  \\
\cmidrule(lr){7-10}\
  & Other & Arch. & Batch & Ep. & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$ & $\eP'$ &  $\eE'$ \\ 
\midrule 
 BEiT  &  & ViT-B16 & 2048 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$  \\
     BEiT  &  & ViT-L16 & 2048 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$  \\
  BEiT  & d: IN22K & ViT-B16 & 2048 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$  \\
   BEiT+ft  & d: IN22K & ViT-B16 & 2048 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$  \\
 \midrule[0.1pt]
 MAE  &   & ViT-B16 & 4096 & 1600 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
 MAE  &   & ViT-L16 & 4096 & 1600 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
 MAE  &   & ViT-H14 & 4096 & 1600 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
  MAE+ft  &   & ViT-B16 & 4096 & 1600 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
 \midrule[0.1pt]
 iBOT  &   & ViT-S16 & 1024 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
iBOT  &   & ViT-B16 & 1024 & 400 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
 \midrule[0.1pt]
 MUGS  &   & ViT-S16 & 1024 & 100 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
 MUGS  &   & ViT-S16 & 1024 & 300 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
  MUGS  &   & ViT-S16 & 1024 & 800 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
 MUGS  &   & ViT-B16 & 1024 & 400 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
 MUGS  &   & ViT-L16 & 640 & 250 & Agg.   & $\eA$ & $\eR$ & $\eP$ &  $\eE$& $\eP'$ &  $\eE'$ 	 \\
\bottomrule
\end{tabular}
\end{center}
\end{scriptsize}
\end{subtable}
\label{table:all_encoders}
\end{table}

